An Evaluated Certification Services System for the German National Root CA - Legally Binding and Trustworthy Transactions in E-Business and E-Government

National Root CAs enable legally binding E-Business and E-Government transactions. This is a report about the development, the evaluation and the certification of the new certification services system for the German National Root CA. We illustrate why a new certification services system was necessary, and which requirements to the new system existed. Then we derive the tasks to be done from the mentioned requirements. After that we introduce the initial situation at the beginning of the project. We report about the very process and talk about some unfamiliar situations, special approaches and remarkable experiences. Finally we present the ready IT system and its impact to E-Business and E-Government.

==> hyphenation.tex <==
\hyphenation{FlexiTRUST} \hyphenation{FlexiPKI}
\hyphenation{Technische} \hyphenation{Darmstadt}

